Safe Domain Randomization via Uncertainty-Aware Out-of-Distribution Detection and Policy Adaptation

Deploying reinforcement learning (RL) policies in real-world involves significant challenges, including distribution shifts, safety concerns, and the impracticality of direct interactions during policy refinement. Existing methods, such as domain randomization (DR) and off-dynamics RL, enhance policy robustness by direct interaction with the target domain, an inherently unsafe practice. We propose Uncertainty-Aware RL (UARL), a novel framework that prioritizes safety during training by addressing Out-Of-Distribution (OOD) detection and policy adaptation without requiring direct interactions in target domain. UARL employs an ensemble of critics to quantify policy uncertainty and incorporates progressive environmental randomization to prepare the policy for diverse real-world conditions. By iteratively refining over high-uncertainty regions of the state space in simulated environments, UARL enhances robust generalization to the target domain without explicitly training on it. We evaluate UARL on MuJoCo benchmarks and a quadrupedal robot, demonstrating its effectiveness in reliable OOD detection, improved performance, and enhanced sample efficiency compared to baselines.

==> figures/data_algorithm.tex <==
\tikzexternaldisable
\begin{algorithm*}[t]
\small
\caption{Balancing replay buffer}\label{alg:data_weight}
\begin{algorithmic}[1]
\BeginBox[fill=gray!20]
\State {\bfseries Require:} 
\Comment{Before balancing}
\Statex \quad ensemble of critics $\{Q_i\}_{i=1}^N$, $\dataset'$ as the repulsive dataset, $\dataset$ as the nominal dataset.
\EndBox
\BeginBox[fill=gray!10]
\For{each $(s, a) \in \dataset' \cup \dataset$} \Comment{Compute variance for every data point}
\State Compute the variance $\sigma^2 (s,a)$ between the critics' outputs $\{Q_i(s,a)\}_{i=1}^N$
\If{$(s, a) \in \dataset'$}
\State Assign weight $w(s, a) \propto \sigma^{-2}(s,a)$ \Comment{Higher weight to ID samples}
\ElsIf{$(s, a) \in \dataset$}
\State Assign weight $w(s, a) \propto \sigma^{2}(s,a)$ \Comment{Higher weight to OOD samples}
\EndIf
\EndFor
\EndBox
\end{algorithmic}
\end{algorithm*}
\tikzexternalenable

